On the Robustness of Removal-Based Feature Attributions

To explain predictions made by complex machine learning models, many feature attribution methods have been developed that assign importance scores to input features. Some recent work challenges the robustness of these methods by showing that they are sensitive to input and model perturbations, while other work addresses this issue by proposing robust attribution methods. However, previous work on attribution robustness has focused primarily on gradient-based feature attributions, whereas the robustness of removal-based attribution methods is not currently well understood. To bridge this gap, we theoretically characterize the robustness properties of removal-based feature attributions. Specifically, we provide a unified analysis of such methods and derive upper bounds for the difference between intact and perturbed attributions, under settings of both input and model perturbations. Our empirical results on synthetic and real-world data validate our theoretical results and demonstrate their practical implications, including the ability to increase attribution robustness by improving the model's Lipschitz regularity.

==> inserts/prior.tex <==
\begin{table}[t]
\centering
\caption{Prior work on feature attribution robustness.}
% \begin{small}
\begin{tabular}{ccc}
\toprule
Paper & Manipulation & Methods \\
\midrule
Ghorbani et al.~\cite{ghorbani2019interpretation} \\
Slack et al.~\cite{slack2020fooling} \\
Anders et al.~\cite{anders2020fairwashing} \\
Dombrowski et al.~\cite{dombrowski2022towards} \\
\midrule
Ours & Input and model & \makecell{Removal-based explanations \\ \cite{zeiler2014visualizing, ribeiro2016should, lundberg2017unified, petsiuk2018rise, chen2020ls}} \\
\bottomrule
\end{tabular}
% \end{small}
\label{tab:prior}
\end{table}

% \textcolor{blue}{Ian: should we list remedies? Maybe not, because that's not our focus}


==> sections/related.tex <==
\input{inserts/prior}

% [Lots of work on explanation methods and theory to support them. For example, unified perspectives on gradient-based methods (Ancona) and removal-based methods.]

Recent work has shown that gradient-based feature attributions for neural networks are susceptible to small input perturbations such that the perturbed attributions differ much from the original attributions \cite{dombrowski2019explanations, ghorbani2019interpretation, kindermans2019reliability}. 

\textbf{Robustness of feature attributions under model perturbation.}

\textbf{Robustness of neural networks.} 

[Some work on robustness for model explanations. Mostly negative results showing high sensitivity to minor changes either in the input or in the model. We distinguish between these types of manipulations and address them separately. We provide a summary of prior works in Table 1 (list works, methods they focused on, manipulations they focused on, suggested remedies). Our work is the first to provide a comprehensive characterization for removal-based explanations, and to show that explanation robustness largely reduces to the well-studied model robustness problem.]

[Lots of work on robustness for model predictions. Adversarial attacks of different kinds, empirical defenses, certified defenses, etc. Lots of work on understanding Lipschitz continuity.]

% \textbf{Manipulating feature attributions.} We distinguish between two types of manipulation for feature attributions. In \textit{input manipulation}, an input is modified with small changes such that the resulting feature attributions drastically differ from the attributions with the unmodified input. In \textit{model manipulation}, a model is slightly modified such that the feature attributions generated from the modified model are drastically different those based on the unmodified model.


